Generalised 6j symbols over the category of $G$-graded vector spaces

Any choice of a spherical fusion category defines an invariant of oriented closed 3-manifolds, which is computed by choosing a triangulation of the manifold and considering a state sum model that assigns a 6j symbol to every tetrahedron in this triangulation. This approach has been generalized to oriented closed 3-manifolds with defect data by Meusburger. In a recent paper, she constructed a family of invariants for such manifolds parametrised by the choice of certain spherical fusion categories, bimodule categories, finite bimodule functors and module natural transformations. Meusburger defined generalised 6j symbols for these objects, and introduces a state sum model that assigns a generalised 6j symbol to every tetrahedron in the triangulation of a manifold with defect data, where the type of 6j symbol used depends on what defect data occur within the tetrahedron. The present work provides non-trivial examples of suitable bimodule categories, bimodule functors and module natural transformation, all over categories of $G$-graded vector spaces. Our main result is the description of module functors in terms of matrices, which allows us to classify these functors when $G$ is a finite cyclic group. Furthermore, we calculate the generalised 6j symbols for categories of $G$-graded vector spaces, (bi-)module categories over such categories and (bi-)module functors.

==> sections/pivotal_old.tex <==
%This coherence datum $\psi^{\otimes}_{X, Y}: Y^*\otimes X^*\to (X\otimes Y)^*$ is defined graphically in \cite[Proposition 2.1.5]{tenscat}
%(see also \cite[Proposition XIV.2.2]{kassel}) as
%%TODO! this is the inverse of the coherence datum! (error also in script)
%
%\begin{center}
%	\begin{tikzpicture}
%		% see TikZ documentation p. 147 for relative coordinates and Bèzier curves
%		
%		\node[morphism, label=0:{$\ident_{X\otimes Y}$}, minimum size=1cm] (I) at (0, 0) {};
%		
%		\draw[thick] (I.north) .. controls +(0, 1) and +(0, 1) .. node[left=1pt, near start] {$X\otimes Y$} ++(2, 0) -- node[right=1pt, near end] {$(X\otimes Y)^*$} ++(0, -3);
%		
%		\draw[thick] (I.south west) .. controls +(0, -1) and +(0, -1) .. node[left=1pt, very near start] {$X$} ++(-1.5, 0) -- node[left=1pt, very near end] {$X^*$} ++(0, 2);
%		\draw[thick] (I.south east) .. controls +(0, -2) and +(0, -2) .. node[right=1pt, very near start] {$Y$} ++(-3.5, 0) -- node[left=1pt, very near end] {$Y^*$} ++(0, 2);
%	\end{tikzpicture}
%\end{center}
%%
%which translates to the algebraic expression
%%
%\begin{multline} \label{eq:coh_*}
%	\psi^{\otimes}_{X, Y} := 
%	\left(\eval_Y^R \otimes \ident_{(X\otimes Y)^*}\right) \circ \left(\ident_{Y^*} \otimes \eval_X^R\otimes \ident_{Y\otimes (X\otimes Y)^*}\right) \circ \left(\ident_{Y^*} \otimes a_{X^*, X, Y}^{-1} \otimes \ident_{(X\otimes Y)^*}\right) \\
%	\circ \left(a_{Y^*, X^*, X\otimes Y} \otimes \ident_{(X\otimes Y)^*}\right) \circ a_{Y^*\otimes X^*, X\otimes Y, (X\otimes Y)^*}^{-1} \circ \left(\ident_{Y^*\otimes X^*} \otimes \coev_{X\otimes Y}^R\right).
%\end{multline}
%%
%Using the graphical calculus, it is easy to check that this turns $*$ into a monoidal functor.
%%
%%A note on the graphical calculus used here: Since $\mathcal C$ need not be a pivotal category, duals are \emph{not} represented by lines oriented upward. The right evaluation and coevaluation are still notated as indicated in section \ref{ssec:graph_fusion}, but 
%
%%The coherence datum of $**$ can now be calculated from $\psi^{\otimes}$:
%
%%TODO! all in wrong direction
%\begin{lemma} \label{lem:coh_**}
%	Let $\psi^{\otimes}$ denote the coherence datum of $*:\mathcal C \to \mathcal C^{op, rev}$. Then $**: \mathcal C \to \mathcal C$ is a monoidal functor with coherence datum
%	\[ \begin{tikzcd}[column sep=large]
%		\phi^{\otimes}_{X, Y} \text{ : } (X \otimes Y)^{**} \ar[r, "\left(\psi^{\otimes}_{X, Y}\right)^*"] & (Y^* \otimes X^*)^* \ar[r, "\left(\psi^{\otimes}_{Y^*, X^*}\right)^{-1}"] & X^{**} \otimes Y^{**}.
%	\end{tikzcd}\]
%\end{lemma}
%\begin{proof}
%	Let $\mathcal C, \mathcal D, \mathcal E$ be arbitrary monoidal categories.
%	\begin{enumerate}
%		\item \label{it:op_mon} Given any monoidal functor $(F, \phi^{\otimes}): \mathcal C \to \mathcal D^{op}$, the functor $F^{op}: \mathcal C^{op} \to \mathcal D$ is monoidal with coherence datum
%		\[ \tilde{\phi}^{\otimes}_{X, Y} = \left(\phi^{\otimes}_{X, Y}\right)^{-1}: F(X\otimes Y) \to FX \otimes FY. \]
%		%checked
%		\item \label{it:rev_mon} Given any monoidal functor $(F, \phi^{\otimes}): \mathcal C\to \mathcal D^{rev}$, the functor $F^{rev}: \mathcal C^{rev} \to \mathcal D$ (identical to $F$ as functor) is monoidal with coherence datum
%		\[ \tilde{\phi}^{\otimes}_{X, Y} = \phi^{\otimes}_{Y, X}: F(Y \otimes X) \to FX \otimes FY. \]
%		%checked
%		\item \label{it:comp_mon}
%		Given monoidal functors $(F, \phi^{\otimes}): \mathcal C\to \mathcal D, (G, \rho^{\otimes}): \mathcal D\to \mathcal E$, their composition $GF$ is a monoidal functor with coherence datum
%		\[ \begin{tikzcd}
%			\phi^{\otimes}_{X, Y} \esccol 
%			GF(X\otimes Y) \ar[r, "G\phi^{\otimes}_{X, Y}"] & G(FX \otimes FY) \ar[r, "\rho^{\otimes}_{FX, FY}"] & GFX \otimes GFY.
%		\end{tikzcd} \]
%		%checked
%	\end{enumerate}
%	It is straightforward to check that these constructions yield monoidal functors. \ref{it:op_mon}. and \ref{it:rev_mon}. imply that $(*)^{op, rev}: \mathcal C^{op, rev}\to \mathcal C$ is a monoidal functor with coherence datum $\tilde\psi_{X, Y}^{\otimes} = (\psi_{Y, X}^{\otimes})^{-1}$.
%	Now apply \ref{it:comp_mon}. to $F=*$ and $G=(*)^{op, rev}$.
%\end{proof}
%
%We now return to the case $\mathcal C = \vectgo$. 
%%The isomorphisms in (\ref{eq:coh_*}) which stem from the adjunctions in Proposition \ref{pro:dual_adj} can be calculated using the formulae for the counits (assume $gh = k$; otherwise the $\Hom$-spaces are trivial):
%%\begin{formarray}{rcl}
%%	\Hom((\delta^g)^* \otimes \delta^k, \delta^h) &\cong &\Hom(\delta^k, \delta^g \otimes \delta^h) \\
%%	\ident &\mapsto &\omega(g, g^{-1}, gh)\, \ident
%%\end{formarray}
%%\begin{formarray}{rcl}
%%	\Hom(\delta^g \otimes \delta^h, \delta^k) &\cong &\Hom(\delta^g, \delta^k \otimes (\delta^h)^*) \\
%%	\ident &\mapsto &\omega^{-1}(g, h, h^{-1})\, \ident
%%\end{formarray}
%%%TODO: align while keeping space between the two parts
%%
%%Setting $X=\delta^g, Y=\delta^h$ in (\ref{eq:coh_*}) now yields
%%\[ \psi^{\otimes}_{g, h} = \omega^{-1}(g, g^{-1}, gh)\, \omega^{-1}(g^{-1}, gh, h^{-1}g^{-1})\, \omega^{-1}(h, h^{-1}, g^{-1}), \]
%%which can be simplified to
%%\[ \psi^{\otimes}_{g, h} = \omega(g, h, h^{-1}g^{-1})\, \omega^{-1}(h, h^{-1}, g^{-1}) \]
%%by using (\ref{eq:3cocycle}) for $(g^{-1}, g, h, h^{-1}g^{-1})$ and $(g, g^{-1}, g, h)$ as well as $\omega(g, g^{-1}, g) = \omega^{-1}(g^{-1}, g, g^{-1})$ (see (\ref{eq:3co_inv})).
%%%TODO: badbox
%%
%\begin{lemma}
%	Pivotal structures on $\vectgo$ are in bijection with characters $\kappa: G\to \units$ of $G$. If $\kappa: G \to \units$ is a character,
%	\[ \beta(g) := \kappa(g)\, \omega^{-1}(g, g^{-1}, g) \]
%	defines a pivotal structure $b$ on $\vectgo$ with $b_g = \beta(g)\, \ident_g$.
%\end{lemma}
%\begin{proof}
%	The coherence datum of $*$ can be determined by setting $X=\delta^g, Y=\delta^h$ in (\ref{eq:coh_*}):
%	%The coherence datum of $*$ as defined in (\ref{eq:coh_*}) is (replace the objects $X$ and $Y$ by $\delta^g$ and $\delta^h$)
%	\begin{multline*}
%		\psi^{\otimes}_{g, h} = \omega(h^{-1}, h, h^{-1}) \, \omega(g^{-1}, g, g^{-1})\, \omega^{-1}(g^{-1}, g, h) \\
%		\omega(h^{-1}, g^{-1}, gh) \, \omega^{-1} (h^{-1}g^{-1}, gh, h^{-1}g^{-1})\ \ident_{h^{-1}g^{-1}}.
%	\end{multline*}
%	By applying the cocycle condition (\ref{eq:3cocycle}) for $(h^{-1}, g^{-1}, gh, h^{-1}g^{-1}), (g^{-1}, g, h, h^{-1}g^{-1})$ and $(h^{-1}, h, h^{-1}, g^{-1})$, this can be simplified to
%	\[ \psi^{\otimes}_{g, h} = \omega(g, h, h^{-1}g^{-1}) \, \omega^{-1}(h, h^{-1}, g^{-1}) \, \ident_{h^{-1}g^{-1}}. \]
%	
%	Hence, by Lemma \ref{lem:coh_**}, the coherence datum of $**$ is
%	\begin{multline*} 
%		\phi^{\otimes}_{g, h} = \left(\psi^{\otimes}_{h^{-1}, g^{-1}}\right)^{-1} \circ \left( \psi^{\otimes}_{g, h} \right)^* = \\ \omega^{-1}(h^{-1}, g^{-1}, gh)\, \omega(g^{-1}, g, h)\, \omega(g, h, h^{-1}g^{-1})\, \omega^{-1}(h, h^{-1}, g^{-1})\, \ident_{gh}.
%	\end{multline*}
%	By applying the cocycle condition (\ref{eq:3cocycle}) for $(g, h, h^{-1}, g^{-1}), (gh, h^{-1}g^{-1}, gh), (g, g^{-1}, g, h)$ and $(g, h, h^{-1}, h)$ we get
%	\[ \phi^{\otimes}_{g, h} = \omega(gh, h^{-1} g^{-1}, gh) \, \omega^{-1}(g, g^{-1}, g)\, \omega^{-1}(h, h^{-1}, h)\, \ident_{gh}. \]
%	
%	We insert $\phi^{\otimes}_{g, h}$ into (\ref{diag:piv_**}) and conclude that $b_g = \beta(g)\, \ident_g$ for $g\in G$ defines a pivotal structure on $\vectgo$ if and only if
%	\[ \beta(gh)\, \omega(gh, h^{-1}g^{-1}, gh)\, = \beta(g)\, \beta(h)\, \omega(g, g^{-1}, g)\, \omega(h, h^{-1}, h). \]
%	This holds if and only if the map $\kappa: G\to \units$ defined by
%	\[ \kappa(g) := \beta(g)\, \omega(g, g^{-1}, g) \]
%	is a character of $G$.
%\end{proof}
%
%We write $\vectgok:= (\vectgo, b)$ with $b_g=\kappa(g)\, \omega(g, g^{-1}, g)\, \ident_g$ for the pivotal category determind by a character $\kappa:G\to \units$.
%%We denote the pivotal category with pivotal structure determined by a charakter $\kappa: G\to \units$ by $\vectgok$.
%%As the pivotal structure is determined by this $\kappa$, we can denote the category $\vectgo$ with pivotal structure $b$ (where $b_g = \beta(g)\,\ident_g$) by $\mathrm{Vec}_G^{\omega, \kappa}$.
%We can now calculate the left evaluation and coevaluation of $\mathrm{Vec}_G^{\omega, \kappa}$ using (\ref{eq:left_eval}) and (\ref{eq:left_coev}). %For convenient reference, we also repeat the right evaluation and coevaluation:
%%
%\begin{formarray}{lcrlcr}
%	\eval_g^R &=& \omega(g^{-1}, g, g^{-1}) \, \ident_1,
%	\hspace*{2em} & \eval_g^L &=& \kappa(g)\, \ident_1 \\
%	\coev_g^R &=& %\phantom{\omega(g^{-1}, g, g^{-1})}
%	\ident_1,
%	\hspace*{2em} &\coev_g^L &=& \beta^{-1}(g)\, \ident_1
%\end{formarray}

==> sections/section07.tex <==
\section{Generalised Turaev-Viro invariants}
\plan{short description}

\plan{definition lens space, calculation of invariant, discussion of results}
